Measurement of the ${}^{136}$Xe two-neutrino double beta decay half-life via direct background subtraction in NEXT

We report a measurement of the half-life of the ${}^{136}$Xe two-neutrino double beta decay performed with a novel direct background subtraction technique. The analysis relies on the data collected with the NEXT-White detector operated with ${}^{136}$Xe-enriched and ${}^{136}$Xe-depleted xenon, as well as on the topology of double-electron tracks. With a fiducial mass of only 3.5 kg of Xe, a half-life of $2.34^{+0.80}_{-0.46}\textrm{(stat)}^{+0.30}_{-0.17}\textrm{(sys)}\times10^{21}~\textrm{yr}$ is derived from the background-subtracted energy spectrum. The presented technique demonstrates the feasibility of unique background-model-independent neutrinoless double beta decay searches.

==> src/authors.tex <==
\author{P.~Novella}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{M.~Sorel}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{A.~Us\'on}
\thanks{Corresponding Author.}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{C.~Adams}
\affiliation{Argonne National Laboratory, Argonne, IL 60439, USA}
%
\author{H.~Almaz\'an}
\affiliation{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\author{V.~\'Alvarez}
\affiliation{Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\author{B.~Aparicio}
\affiliation{Department of Organic Chemistry I, University of the Basque Country (UPV/EHU), Centro de Innovaci\'on en Qu\'imica Avanzada (ORFEO-CINQA), San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{A.I.~Aranburu}
\affiliation{Department of Applied Chemistry, Universidad del Pais Vasco (UPV/EHU), Manuel de Lardizabal 3, San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{L.~Arazi}
\affiliation{Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\author{I.J.~Arnquist}
\affiliation{Pacific Northwest National Laboratory (PNNL), Richland, WA 99352, USA}
%
\author{S.~Ayet}
\affiliation{II. Physikalisches Institut, Justus-Liebig-Universitat Giessen, Giessen, Germany}
%
\author{C.D.R.~Azevedo}
\affiliation{Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro, Campus de Santiago, Aveiro, 3810-193, Portugal}
%
\author{K.~Bailey}
\affiliation{Argonne National Laboratory, Argonne, IL 60439, USA}
%
\author{F.~Ballester}
\affiliation{Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\author{J.M.~Benlloch-Rodr\'{i}guez}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{F.I.G.M.~Borges}
\affiliation{LIP, Department of Physics, University of Coimbra, Coimbra, 3004-516, Portugal}
%
\author{S.~Bounasser}
\affiliation{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\author{N.~Byrnes}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{S.~C\'arcel}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{J.V.~Carri\'on}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{S.~Cebri\'an}
\affiliation{Centro de Astropart\'iculas y F\'isica de Altas Energ\'ias (CAPA), Universidad de Zaragoza, Calle Pedro Cerbuna, 12, Zaragoza, E-50009, Spain}
%
\author{E.~Church}
\affiliation{Pacific Northwest National Laboratory (PNNL), Richland, WA 99352, USA}
%
\author{C.A.N.~Conde}
\affiliation{LIP, Department of Physics, University of Coimbra, Coimbra, 3004-516, Portugal}
%
\author{T.~Contreras}
\affiliation{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\author{F.P.~Coss\'io}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%\affiliation{Ikerbasque (Basque Foundation for Science), Bilbao, E-48009, Spain}
%
\author{A.A.~Denisenko}
\affiliation{Department of Chemistry and Biochemistry, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{G.~D\'iaz}
\affiliation{Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%
\author{J.~D\'iaz}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{T.~Dickel}
\affiliation{II. Physikalisches Institut, Justus-Liebig-Universitat Giessen, Giessen, Germany}
%
\author{J.~Escada}
\affiliation{LIP, Department of Physics, University of Coimbra, Coimbra, 3004-516, Portugal}
%
\author{R.~Esteve}
\affiliation{Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\author{A.~Fahs}
\affiliation{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\author{R.~Felkai}
\affiliation{Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\author{L.M.P.~Fernandes}
\affiliation{LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\author{P.~Ferrario}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%\affiliation{Ikerbasque (Basque Foundation for Science), Bilbao, E-48009, Spain}
%
\author{A.L.~Ferreira}
\affiliation{Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro, Campus de Santiago, Aveiro, 3810-193, Portugal}
%
\author{F.W.~Foss}
\affiliation{Department of Chemistry and Biochemistry, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{E.D.C.~Freitas}
\affiliation{LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\author{Z.~Freixa}
\affiliation{Department of Applied Chemistry, Universidad del Pais Vasco (UPV/EHU), Manuel de Lardizabal 3, San Sebasti\'an / Donostia, E-20018, Spain}
%\affiliation{Ikerbasque (Basque Foundation for Science), Bilbao, E-48009, Spain}
%
\author{J.~Generowicz}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{A.~Goldschmidt}
\affiliation{Lawrence Berkeley National Laboratory (LBNL), 1 Cyclotron Road, Berkeley, CA 94720, USA}
%
\author{J.J.~G\'omez-Cadenas}
\thanks{NEXT Co-spokesperson.}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
\affiliation{Ikerbasque (Basque Foundation for Science), Bilbao, E-48009, Spain}
%
\author{R.~Gonz\'alez}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{D.~Gonz\'alez-D\'iaz}
\affiliation{Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%
\author{R.~Guenette}
\affiliation{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\author{R.M.~Guti\'errez}
\affiliation{Centro de Investigaci\'on en Ciencias B\'asicas y Aplicadas, Universidad Antonio Nari\~no, Sede Circunvalar, Carretera 3 Este No.\ 47 A-15, Bogot\'a, Colombia}
%
\author{J.~Haefner}
\affiliation{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\author{K.~Hafidi}
\affiliation{Argonne National Laboratory, Argonne, IL 60439, USA}
%
\author{J.~Hauptman}
\affiliation{Department of Physics and Astronomy, Iowa State University, Ames, IA 50011-3160, USA}
%
\author{C.A.O.~Henriques}
\affiliation{LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\author{J.A.~Hernando~Morata}
\affiliation{Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%
\author{P.~Herrero-G\'omez}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%\affiliation{Centro de F\'isica de Materiales (CFM), CSIC \& Universidad del Pais Vasco (UPV/EHU), Manuel de Lardizabal 5, San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{V.~Herrero}
\affiliation{Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\author{J.~Ho}
\affiliation{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\author{Y.~Ifergan}
\affiliation{Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\author{B.J.P.~Jones}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{M.~Kekic}
\affiliation{Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%
\author{L.~Labarga}
\affiliation{Departamento de F\'isica Te\'orica, Universidad Aut\'onoma de Madrid, Campus de Cantoblanco, Madrid, E-28049, Spain}
%
\author{A.~Laing}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{P.~Lebrun}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
%
\author{D.~Lopez Gutierrez}
\affiliation{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\author{N.~L\'opez-March}
\affiliation{Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\author{M.~Losada}
\affiliation{Centro de Investigaci\'on en Ciencias B\'asicas y Aplicadas, Universidad Antonio Nari\~no, Sede Circunvalar, Carretera 3 Este No.\ 47 A-15, Bogot\'a, Colombia}
%
\author{R.D.P.~Mano}
\affiliation{LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\author{J.~Mart\'in-Albo}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{A.~Mart\'inez}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{G.~Mart\'inez-Lema}
\affiliation{Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\author{M.~Mart\'inez-Vara}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{A.D.~McDonald}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{Z.E.~Meziani}
\affiliation{Argonne National Laboratory, Argonne, IL 60439, USA}
%
\author{K.~Mistry}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{F.~Monrabal}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
\affiliation{Ikerbasque (Basque Foundation for Science), Bilbao, E-48009, Spain}
%
\author{C.M.B.~Monteiro}
\affiliation{LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\author{F.J.~Mora}
\affiliation{Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\author{J.~Mu\~noz Vidal}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{K.~Navarro}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{D.R.~Nygren}
\thanks{NEXT Co-spokesperson.}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{E.~Oblak}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{M.~Odriozola-Gimeno}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{B.~Palmeiro}
\affiliation{Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{A.~Para}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
%
\author{J.~P\'erez}
\affiliation{Laboratorio Subterr\'aneo de Canfranc, Paseo de los Ayerbe s/n, Canfranc Estaci\'on, E-22880, Spain}
%
\author{M.~Querol}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{A.~Raymond}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{A.B.~Redwine}
\affiliation{Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\author{J.~Renner}
\affiliation{Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%
\author{L.~Ripoll}
\affiliation{Escola Polit\`ecnica Superior, Universitat de Girona, Av.~Montilivi, s/n, Girona, E-17071, Spain}
%
\author{I.~Rivilla}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%\affiliation{Ikerbasque (Basque Foundation for Science), Bilbao, E-48009, Spain}
%
\author{Y.~Rodr\'iguez Garc\'ia}
\affiliation{Centro de Investigaci\'on en Ciencias B\'asicas y Aplicadas, Universidad Antonio Nari\~no, Sede Circunvalar, Carretera 3 Este No.\ 47 A-15, Bogot\'a, Colombia}
%
\author{J.~Rodr\'iguez}
\affiliation{Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\author{C.~Rogero}
\affiliation{Centro de F\'isica de Materiales (CFM), CSIC \& Universidad del Pais Vasco (UPV/EHU), Manuel de Lardizabal 5, San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{L.~Rogers}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{B.~Romeo}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%\affiliation{Laboratorio Subterr\'aneo de Canfranc, Paseo de los Ayerbe s/n, Canfranc Estaci\'on, E-22880, Spain}
%
\author{C.~Romo-Luque}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\author{F.P.~Santos}
\affiliation{LIP, Department of Physics, University of Coimbra, Coimbra, 3004-516, Portugal}
%
\author{J.M.F. dos~Santos}
\affiliation{LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\author{A.~Sim\'on}
\affiliation{Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\author{C.~Stanford}
\affiliation{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\author{J.M.R.~Teixeira}
\affiliation{LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\author{P.~Thapa,}
\affiliation{Department of Chemistry and Biochemistry, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{J.F.~Toledo}
\affiliation{Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\author{J.~Torrent}
\affiliation{Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%
\author{J.F.C.A.~Veloso}
\affiliation{Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro, Campus de Santiago, Aveiro, 3810-193, Portugal}
%
\author{T.T.~Vuong}
\affiliation{Department of Chemistry and Biochemistry, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{R.~Webb}
\affiliation{Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843-4242, USA}
%
\author{R.~Weiss-Babai}
\thanks{On leave from Soreq Nuclear Research Center, Yavneh, Israel.}
\affiliation{Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\author{J.T.~White}
\thanks{Deceased.}
\affiliation{Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843-4242, USA}
%
\author{K.~Woodruff}
\affiliation{Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\author{N.~Yahlali}
\affiliation{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%

